SimPB++: Simultaneously Detecting 2D and 3D Objects from Multiple Cameras

Simultaneous perception of 2D objects in perspective view and 3D objects in Bird's Eye View (BEV) is challenging for multi-camera autonomous driving. Existing two-stage pipelines use 2D results only as a one-time cue for 3D detection. We propose SimPB++, which simultaneously detects 2D objects in perspective and 3D objects in BEV from multiple cameras. It unifies both tasks into an end-to-end model with a hybrid decoder architecture, coupling multi-view 2D and 3D decoders interactively. Two novel modules enable deep interaction: Dynamic Query Allocation adaptively assigns 2D queries to 3D candidates, and Adaptive Query Aggregation refines 3D representations using multi-view 2D features, forming a cyclic 3D-2D-3D refinement. For multi-view 2D detection, we use Query-group Attention for intra-group communication. We also design a Crop-and-Scale strategy for long-range perception and a Propagating Denoising strategy with an auxiliary RoI detector. SimPB++ supports mixed supervision with 2D-only and fully annotated data, reducing reliance on expensive 3D labels. Experiments show state-of-the-art performance on nuScenes for both tasks and strong long-range detection (up to 150m) on Argoverse2.

==> table/2_nuscenes_test.tex <==
\begin{table*}[t]
\centering
\caption{Comparison results of 3D detection on nuScenes test dataset. \hlr{Website Stuck, Cannot Evaluate Test!!!}}

\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{@{}l|c|c|cc|ccccc@{}}
    \toprule
    Method  & \ \, Backbone\ \,  & \ \, Resolution\ \,& \ mAP$\uparrow$\,  & \,NDS$\uparrow$\ & \,mATE\,$\downarrow$ & \,mASE\,$\downarrow$ & \,mAOE\,$\downarrow$ & \,mAVE\,$\downarrow$ & \,mAAE\,$\downarrow$ \\
    \midrule
    StreamPETR\cite{StreamPETR}  & V2-99 &$1600\times 640$& 0.550& 0.636& 0.479& 0.239& 0.317& 0.241& 0.119 \\
    SparseBEV\cite{SparseBEV}    & V2-99 &$1600\times 640$& 0.556& 0.636& 0.485& 0.244& 0.332& 0.246& 0.117 \\
    Sparse4Dv2\cite{Sparse4Dv2}  & V2-99 &$1600\times 640$& 0.556& 0.638& 0.462& 0.238& 0.328& 0.264& 0.115 \\
    BEVNext\cite{BEVNeXt}        & V2-99 &$1600\times 640$& 0.557& 0.642& \textbf{0.409}& 0.241& 0.352& 0.233& 0.129 \\    
    DynamicBEV\cite{DynamicBEV}  & V2-99 &$1600\times 640$& 0.566& 0.648& 0.486& 0.245& 0.343& 0.240& \textbf{0.115} \\  
    Sparse4Dv3\cite{Sparse4Dv3}  & V2-99 &$1600\times 640$& 0.570& 0.656& 0.412& \textbf{0.236}& 0.312& 0.210& 0.117 \\  
    \rowcolor{gray!15}
    SimPB                        & V2-99 &$1600\times 640$& \textbf{0.571}& \textbf{0.660}& 0.419& 0.239& \textbf{0.262}& \textbf{0.201}& 0.133  \\
    \rowcolor{gray!15}
    \hlr{SimPB++}                & V2-99 &$1600\times 640$& & & & & & & \\
    \bottomrule
\end{tabular}
}
\label{tab:nus_test}
\end{table*}



==> table/9_ablation_integration.tex <==
\begin{table}
\centering
\caption{Integrate our SimPB to other methods.}
\begin{tabular}{l|llc}
    \toprule
    Method \qquad \qquad \qquad  & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\ \\
    \midrule
    DETR3D~\cite{DETR3D}         & \ 0.258   & 0.306   \\
    \rowcolor{gray!15}
    DETR3D-SimPB                 & \ 0.282 (+\hlr{0.024})  & 0.358 (+\hlr{0.052}) \\
    \midrule
    Sparse4Dv2~\cite{Sparse4Dv2} & \ 0.367  & 0.450  \\
    \rowcolor{gray!15}
    Sparse4Dv2-SimPB \           & \ 0.398 (+\hlr{0.031})  & 0.480 (+\hlr{0.030}) \\
    \bottomrule
\end{tabular}
\label{tab:ablation_integrate}
\end{table}


==> table/analysis_scale_crop.tex <==
\begin{table}
\centering
\caption{\hlr{The ablation of the efficiency on a NVIDIA 4090 GPU, where the nus and av2 denote the NuScenes and Argoverse2 dataset, respectively.}}
\scalebox{0.75}{
\begin{tabular}{l|l|llc|c}
    \toprule
  Dataset &  Method  & scale-and-crop & mAP& NDS/CDS \\
    \midrule
    nus &SimPB      & \checkmark &            12.0 \\
    nus &SimPB++    & \checkmark &            16.0 \\
    \midrule
    av2 &SimPB      & \checkmark &            7.8 \\
    av2 &SimPB++    & \checkmark &            10.5 \\
    \bottomrule
\end{tabular}
}
\label{tab:analysis_scale_crop}
\end{table}

==> table/merge_table_5_6.tex <==
\begin{table*}[t]
\begin{floatrow}
\capbtabbox{
\scalebox{0.8}{
  \begin{tabular}{l|cc}
    \toprule
    Allocation Strategy & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\  \\
    \midrule
    Uniform                               & 0.365    & 0.474        \\
    Object Center                         & 0.410    & 0.515        \\
    Object Center + Front-Rear Point      & 0.414    & 0.520        \\
    \rowcolor{gray!15}
    Object Center + Anchor Corner \qquad  & \textbf{0.421}    & \textbf{0.527}        \\
    \bottomrule
\end{tabular}
}}
{
\caption{Ablation studies on query allocation mechanism.}
\label{tab:ablation_allocation}
}
\capbtabbox{
\scalebox{0.8}{
\begin{tabular}{l|cc}
    \toprule
    Aggregation Strategy \ & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\  \\
    \midrule
    Cross-Attention                \  & 0.365     & 0.474    \\
    Cross-Attention + Supervision  \  & 0.399     & 0.495    \\
    Query Fusion                   \  & 0.389     & 0.489    \\
    \rowcolor{gray!15}
    Query Fusion + Supervision     \  & \textbf{0.421}     & \textbf{0.527}    \\
    \bottomrule
\end{tabular}
}
}
{
\caption{Ablation studies on query aggregation mechanism.}
\label{tab:ablation_aggregation}
 \small
}
\end{floatrow}
\end{table*}

==> table/merge_table_7_8.tex <==
\begin{table*}[t]
\begin{floatrow}
\capbtabbox{
\scalebox{0.851}{
\begin{tabular}{@{}l|ccc@{}}
    \toprule
    \ \ $\lambda_{alpha}$   & \ mAP$\uparrow$\,  & \,NDS$\uparrow$ \, & \ mAOE$\downarrow$ \\
    \midrule
    \ \ -            & 0.421          & 0.514 & 0.611  \\
    \ \ 0.25         & \textbf{0.425} & 0.519 & 0.582  \\
    \rowcolor{gray!15}
    \ \ 0.50         & 0.421 & \textbf{0.527} & 0.492  \\
    \ \ 1.00         & 0.418 & 0.523 & \textbf{0.465}  \\
    
    \bottomrule
\end{tabular}
}
}{
\caption{The ablation studies of camera observation loss.}
\label{tab:ablation_loss}
}
\capbtabbox{
\scalebox{0.79}{
\begin{tabular}{l|llc}
    \toprule
    Method \qquad \qquad \qquad  & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\ \\
    \midrule
    DETR3D~\cite{DETR3D}         & \ 0.258   & 0.306   \\
    \rowcolor{gray!15}
    DETR3D-SimPB                 & \ 0.282 (+\hlb{0.024})  & 0.358 (+\hlb{0.052}) \\
    \midrule
    Sparse4Dv2~\cite{Sparse4Dv2} & \ 0.367  & 0.450  \\
    \rowcolor{gray!15}
    Sparse4Dv2-SimPB \           & \ 0.398 (+\hlb{0.031})  & 0.480 (+\hlb{0.030}) \\
    \bottomrule
\end{tabular}
}
}
{
\caption{Comparison of SimPB with different 3D detectors.}
\label{tab:ablation_integrate}
 \small
}
\end{floatrow}
\end{table*}

==> table/sup_ablation_encoder.tex <==
\begin{table}[htbp]
\centering
\caption{
%The ablation studies of encoder layer.
Impact of encoder layer of SimPB.
}
\scalebox{0.8}{
\begin{tabular}{@{}c|ccccc@{}}
    \toprule
    \ Encoder layers \  & \ mAP$\uparrow$\,  & \,NDS$\uparrow$ \, & \,$\text{AP}_{2d}\uparrow$ \,&  FPS$\uparrow$ \ & \,Memory(G)\,$\downarrow$ \\
    \midrule
    \ - \        & 0.412 & 0.519 & 0.211 & 12.9 &  10.64\\
    \rowcolor{gray!15}
    \ 1 \        & 0.421 & 0.527 & 0.217 & 10.9 &  14.46\\
    \ 2 \        & 0.425 & 0.529 & 0.220 & 9.0  &  17.89\\
    \ 3 \        & 0.432 & 0.536 & 0.222 & 7.9  &  21.07\\ 
    \ 4 \        & 0.439 & 0.545 & 0.224 & 6.1  &  23.94\\ 
    \bottomrule
\end{tabular}
}
\label{tab:sup_ablation_encoder}
\end{table}

==> table/sup_runtime_comparision.tex <==
\begin{table}[htbp]
\centering
\caption{
%Runtimes comparisons with state-of-art works.
%Comparison of inference speed with previous approaches.
Comparison of inference speeds.
}
\scalebox{0.7}{
\begin{tabular}{@{}l|cc|c@{}}
    \toprule
    \ Method \  & \, Backbone\,  & \, Resolution \, & \, FPS$\uparrow$ \,\\
    \midrule
    \ MV2D\cite{MV2D}             \  & ResNet50  & $704 \times 256$ & 9.5   \\
    \ StreamPETR\cite{StreamPETR} \  & ResNet50  & $704 \times 256$ & 27.1   \\
    \ Sparse3Dv3\cite{Sparse4Dv3} \  & ResNet50  & $704 \times 256$ & 19.8   \\
    \rowcolor{gray!15}
    \ SimPB \                        & ResNet50  & $704 \times 256$ & 10.9   \\
    \midrule
    \ MV2D\cite{MV2D}             \  & ResNet101  & $1408 \times 512$ & 3.9   \\
    \ StreamPETR\cite{StreamPETR} \  & ResNet101  & $1408 \times 512$ & 6.4   \\
    \ Sparse3Dv3\cite{Sparse4Dv3} \  & ResNet101  & $1408 \times 512$ & 8.2   \\
    \rowcolor{gray!15}
    \ SimPB                       \  & ResNet101  & $1408 \times 512$ & 7.1   \\
    \bottomrule
\end{tabular}
}
\label{tab:sup_runtimes_comparision}
\end{table}






